Verifying Security Protocols using Dynamic Strategies

Current formal approaches have been successfully used to find design flaws in many security protocols. However, it is still challenging to automatically analyze protocols due to their large or infinite state spaces. In this paper, we propose a novel framework that can automatically verifying security protocols without any human intervention. Experimental results show that SmartVerif automatically verifies security protocols that cannot be automatically verified by existing approaches. The case study also validates the effectiveness of our dynamic strategy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> backup.tex <==

Unfortunately, although formal analysis has been successful in finding design flaws in security protocols,
there remains a challenge that existing verification tools \cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05},
\cite{DBLP:conf/csfw/Blanchet01,DBLP:conf/fosad/EscobarMM07,DBLP:conf/cav/MeierSCB13,DBLP:conf/csfw/ArapinisRR11,DBLP:conf/sp/KremerK14} do not support the fully automatically analysis of security protocols, especially stateful security protocols with unbounded sessions \cite{PKCS11standard,yubikeymanual,DBLP:conf/crypto/GarayJM99,DBLP:conf/csfw/ArapinisRR11,DBLP:conf/ccs/Modersheim10}.
% The incomplete support of fully automatically analyzing stateful protocols is caused by the simple and duplicated proof strategy of current verification tools in multiple verification processes.
Automated verification of security properties in protocols in the bounded-session model (where a session is one execution of a protocol role by a single principal) has been shown to be decidable \cite{DBLP:journals/tcs/RusinowitchT03} and several bounded-session automated verification tools \cite{DBLP:conf/csfw/ArapinisRR11,DBLP:conf/csfw/BruniMNN15} which specify the maximum number of sessions that can be generated in a search exist. 
StatVerif tool by Arapinis \etal \cite{DBLP:conf/csfw/ArapinisRR11} proposes an extension of the applied pi calculus which can be automatically analyzed by the ProVerif tool \cite{DBLP:conf/csfw/Blanchet01}. However, Statverif can only handle a finite number of protocol sessions.
When analyzing an contract signing protocol \cite{DBLP:conf/crypto/GarayJM99} this appeared to be a limitation and only the status of a single contract was modeled, providing a manual proof to justify the correctness of this abstraction. 
The AVISPA platform \cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05} bounds the number of steps of honest agents which is often fine for finding attacks, but gives limited guarantees for verification.
This can work well for protocols based on public key cryptography, but runs into problems with several authentication and contract protocols \cite{DBLP:conf/crypto/GarayJM99,PKCS11standard,yubikeymanual}. 

Moreover, a number of unbounded-session automated verification tools \cite{DBLP:conf/sp/KremerK14,DBLP:conf/cav/MeierSCB13,DBLP:conf/csfw/Blanchet01} either make use of abstraction to enforce decidability, or allow for the possibility of non-termination.
% StatVerif tool by Arapinis \etal \cite{DBLP:conf/csfw/ArapinisRR11} propose an extension of the applied pi calculus, which is translated to Horn clauses and analyzed by the ProVerif tool. Their translation is sound but limits the scope of protocols that can be analyzed. Moreover, StatVerif can only handle a finite number of protocol sessions and is limited to the verification of secrecy properties.
For example, the ProVerif tool \cite{DBLP:conf/csfw/Blanchet01} uses an abstraction that encodes protocols in Horn clauses to avoid the exploration of the state space of a verifications system. 
The abstraction is efficient because it avoids the common state-explosion of protocol verification and it does not require a limitation to bounded sessions. 
While this works fine for many protocols \cite{DBLP:conf/csfw/KustersT09,DBLP:conf/post/ChevalB13,DBLP:conf/post/ChothiaSS15}, it lacks support for protocols which maintain long term global states \cite{DBLP:conf/crypto/GarayJM99,PKCS11standard,yubikeymanual}. 
This state is not local to a session: if one session updates the state, then it is updated for other sessions too. 
For these stateful protocols, ProVerif models an ever-increasing set of facts representing attacker knowledge, and is not able to associate those facts with the states in which they arose. 
For this reason, the tool typically reports many false attacks \cite{DBLP:conf/csfw/ArapinisRR11,DBLP:conf/csfw/BruniMNN15}. 


Another verification approach that supports the automated verification of protocols with unbounded sessions is the Tamarin prover \cite{DBLP:conf/cav/MeierSCB13,DBLP:conf/sp/KremerK14}. 
Instead of abstraction techniques, it uses backward search and lemmata that allow to cut of search to cope with the infinite state spaces. 
The benefit of Tamarin \cite{DBLP:conf/cav/MeierSCB13} and related tools \cite{DBLP:conf/sp/KremerK14} is a great amount of flexibility in formalising relationships between data that cannot be captured by a particular abstraction approach.
However it comes at the price of loosing automation, \ie, that the user has to supply insight into the problem by proving auxiliary lemmata.
Even for quite simple stateful protocols \cite{DBLP:conf/ccs/Modersheim10}, such lemmata have to be supplied by the user to achieve termination.

==> old-framework.tex <==
%!TEX root =s-verifywithrl.tex
\section{Framework} % (fold)
\label{sec:framework}

In this section, we explain how our work automates the analysis of security protocols using Deep Q Network. 
We provide a framework in \Cref{fig:framework}.

As shown in \Cref{sec:preliminaries}, the verification of protocol in tamarin prover is the process of choosing one applicable rule from a proof state and applying these rules to generate new proof states.
Based on this observation, we modify tamarin prover to get all the applicable constraint solving rules and proof states.
Given a protocol model as input, we collect these data and use a tree structure to store it.
The root node of tree is the proof target and each node constains data of a constraint solving rule and its proof state.
Once a applicable rule is applied to the proof state, new nodes which represent the new proof state and new applicable rules will be the children of current node.
Using tree structure, tamarin prover's complicate verification process is simplified and we can build an path selection and verification system to interactive with the verification tree and the network.
In general, given the verification tree, the system chooses a path from the tree with the guidance of Deep Q Network and verifies the path using tamarin prover.
The proof results outputted by tamarin prover can be used as the reward of the network's past choices and the network can learn and optimize itself with this reward.

In detail, our system contains two parts:

\subsection{Tree construction and update module}

Given the protocol model as input, the Tree Construction submodule collects the applicable rules and their coresponding proof states and constructs a verification tree.
Since the modified tamarin prover only chooses one rule in a proof state, the generated tree is not complete and nodes representing the unchosen rules do not have a child.
Instead of repetitively performing collecting and combining the rules, we use a more efficent strategy to get the complete verification tree.
Firstly, we use the Path Generation submodule to search for leaf nodes and generate proof paths from root node to these leaf nodes.
Then, the Subtree Construction submodule passes the proof paths to modified tamarin prover and collect the rules and proof states and construct a subtree.
Given the verification tree and subtree which contains new nodes, the Tree Merger submodule combines these two trees and generate a complete verification tree. 
Since the verification tree can be extremely large in complicated stateful protocols, we set a global variable to bound the depth of the tree, which initially is 5.
Once the tree does not have any leaf nodes whose depth is smaller than the bounded depth, it is passed to the next Path selection and verification module.


\subsection{Path selection and verification module}

To perform a more flexible and smart verification of protocol, the Path Selection System interacts with Deep Q Network to repeatedly select a child node from root node of the verification tree and generate a corresponding proof path.
Given a node and its corresponding proof state, Deep Q Network computes each child's Q value, which means the possiblity of a successful verification, and outputs the action which has the largest Q value.
The Path Selecton System chooses the child node corresponding to the action and repeatedly performing this selction with the network until it encounters a leaf node.
The chosen nodes constitute a proof path and this path is passed to the Proof Verification submodule to verify whether the choice of the network is right.
The Proof Verification submodule converts the proof path to the proof steps which tamarin prover can verify.

1) If loops exist in these proof steps, which may cause a non-termination problem, the Proof Verification submodule gives these steps a negative reward value.

2) If the proof target is proved, the network gives these proof steps a positive reward value.

Under these two circumstances, we stores these rewards to a memory for network to learn and resets the verification tree to begin a new verification episode.

3) If the tamarin prover outputs a 'incomplete proof' result which means the given proof steps are not complete, the Path Transponder submodule passes the proof paths to the Tree Construction submodule to generate a deeper verification tree.
Under this circumstance, we add the global bounded depth by 5.




% In this section, we introduce a general framework to fully automatically verify security protocols with Deeq Q Learning. In general, the framework contains two parts: 

% 1) Constructing a verification tree of the protocol. 

% After modelling the security protocol in tamarin prover, we perform automated random proof search in tamarin's automated mode to generate the verification tree of the protocol.
% The roof node of the tree is the proof target and each node in the tree contains data structure presenting current proof state. 
% One node is the other's parent if a proof method is applied in the constraint system.
% Only the subpath proof of one theorem is needed to complete the proof of the theorem; and the case proof needs to prove all its subpaths. If all the paths are proved, The proof of the case is completed, otherwise it proves wrong. The parent and child nodes in the tree constitute proof dependencies. Using the theorem tree, the final proof target is disassembled into a series of subproof tasks (\ie, nodes in the tree), and the proof process is transformed into automatic proof of the independent theorems and the automatic reasoning process of the nodes between the theorems, thereby reducing the state space complexity of protocol proving.

% Tamarin proves lemmas using constraint solving. Namely, it refines the knowledge it has about the property and the protocol (called a constraint system) until it can either conclude that the property holds in all possible cases, or until it finds a counterexample to the lemma.

% On the right, we now have the possible proof steps at the top, and the current state of the constraint system just below (which is empty, as we have not started the proof yet). A proof always starts with either a simplification step (1. simplify), which translates the lemma into an initial constraint system that needs to be resolved, or an induction setup step (2. induction), which generates the necessary constraints to prove the lemma using induction on the length of the trace. Here we use the default strategy, i.e., a simplification step by clicking on 1. simplify, to obtain the following screen:

% Tamarin has now translated the lemma into a constraint system. Since Tamarin looks for counterexamples to the lemma, it looks for a protocol execution that contains a SessKeyC( S, k ) and a K( k ) action, but does not use an LtkReveal( S ). This is visualized in the graph as follows. The only way of getting a SessKeyC( S, k ) action is using an instance of the Client\_2 rule on the left, and the K( k ) rule is symbolized on the right using a round box (adversary reasoning is always visualized using round boxes). Just below the graph, the formula

% $formulas: ∀ \#r. (LtkReveal( S ) @ \#r) ⇒ ⊥$

% now states that any occurrence of LtkReveal( S ) will lead to a contradiction.

% To finish the proof, we can either continue manually by selecting the constraint to resolve next, or by calling the autoprove command, which selects the next steps based on a heuristic. Here we have two constraints to resolve: Client\_1( S, k ) and KU( k ), both of which are premises for the rules in the unfinished current constraint system.

% Note that that the proof methods in the Tamarin are sorted according to the same heuristic as is used by the autoprove command. Any proof found by always selecting the first proof method will be identical to the one constructed by the autoprove command. However, because the general problem is undecidable, the algorithm may not terminate for every protocol and property.

% 2) learning the proof strategy using DQN. 

% We build a Deep Q Network based on the features from historical proof data and train it to find the most appropriate proof path in the verification tree.

==> old_introduction.tex <==
%!TEX root =s-verifywithrl.tex
\section{Introduction} % (fold)
\label{sec:introduction}

% Motivation
Security protocols aim at providing securing communications on insecure networks by applying cryptographic primitives.
However, the design of security protocols is particularly error-prone.
Design flaws have been for instance discovered in the Google Single Sign On Protocol \cite{DBLP:conf/ccs/ArmandoCCCT08}, in commercial security tokens implementing the PKCS\#11 standard 
\cite{DBLP:conf/ccs/BortolozzoCFS10}, and one may also recall Lowe’s attack \cite{DBLP:conf/tacas/Lowe96} on the Needham-Schroeder public key protocol 17 years after its publication.
These findings have made the verification of security protocols a very active research area since the 1990s.

% 加上avispa
During the last 30 years, many research efforts
\cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05,DBLP:conf/csfw/Blanchet01,DBLP:conf/fosad/EscobarMM07,DBLP:conf/cav/MeierSCB13}
were spent on designing techniques to model and analyze protocols.
The earliest protocol analysis tools, such as the Interrogator \cite{DBLP:journals/tse/MillenCF87} and the NRL Protocol Analyzer \cite{DBLP:conf/csfw/Meadows96} could be used to verify security properties specified in temporal logic. 
Later, researchers used generic model checking tools to analyze protocols, such as FDR \cite{DBLP:conf/tacas/Lowe96} and later Murphi \cite{mitchell1997automated}. 
More recently the focus has been on model checking tools developed specifically for security protocol analysis, such as Blanchet’s ProVerif \cite{DBLP:conf/csfw/Blanchet01}, the AVISPA tool \cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05}, Maude-NPA \cite{DBLP:conf/fosad/EscobarMM07} and tamarin prover \cite{DBLP:conf/cav/MeierSCB13}.
% In particular ProVerif \cite{DBLP:conf/csfw/Blanchet01} relies on an abstraction that encodes protocols in first-order Horn clauses, which makes the tool extremely efficient for verifying an unbounded number of protocol sessions.
% The Maude-NPA tool \cite{DBLP:journals/tcs/EscobarMM06} employs various state space reduction techniques \cite{DBLP:conf/esorics/EscobarMM08} to ignore some interleavings, which is effective for several security protocols. 
% Instead of abstraction techniques, tamarin prover \cite{DBLP:conf/cav/MeierSCB13} uses backward search and lemmata that allow to cut of search to cope with the infinite state spaces. 
There has also been hand proofs aimed at particular protocols. In \cite{DBLP:journals/jcs/DelauneKS10}, Delaune \etal show by a dedicated hand proof that for analyzing PKCS\#11 one may bound the message size. 
Their analysis still requires to artificially bound the number of keys.
Similarly in spirit, Delaune \etal \cite{DBLP:conf/csfw/DelauneKRS11} give a dedicated result for analyzing protocols based on the TPM and its registers. However, the number of reboots (which reinitialize registers) needs to be limited.
Guttman \cite{DBLP:journals/jar/Guttman12} also extended the space model by adding support for Wang\'s fair exchange protocol \cite{DBLP:journals/jcs/Wang06}. The extended model has been used for analyzing the protocol by hand. 


Unfortunately, although formal analysis has been successful in finding design flaws in security protocols,
there remains a challenge that existing verification tools \cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05},
\cite{DBLP:conf/csfw/Blanchet01,DBLP:conf/fosad/EscobarMM07,DBLP:conf/cav/MeierSCB13,DBLP:conf/csfw/ArapinisRR11,DBLP:conf/sp/KremerK14} do not support the fully automatically analysis of security protocols, especially stateful security protocols \cite{PKCS11standard,yubikeymanual,DBLP:conf/crypto/GarayJM99,DBLP:conf/csfw/ArapinisRR11,DBLP:conf/ccs/Modersheim10}.
% The incomplete support of fully automatically analyzing stateful protocols is caused by the simple and duplicated proof strategy of current verification tools in multiple verification processes.
Indeed, automated verification of security properties in protocols in the bounded-session model (where a session is one execution of a protocol role by a single principal) has been shown to be decidable \cite{DBLP:journals/tcs/RusinowitchT03} and several bounded-session automated verification tools \cite{DBLP:conf/csfw/ArapinisRR11,DBLP:conf/csfw/BruniMNN15} which specify the maximum number of sessions that can be generated in a search exist. 
StatVerif tool by Arapinis \etal \cite{DBLP:conf/csfw/ArapinisRR11} proposes an extension of the applied pi calculus which can be automatically analyzed by the ProVerif tool \cite{DBLP:conf/csfw/Blanchet01}. However, Statverif can only handle a finite number of protocol sessions.
When analyzing an contract signing protocol \cite{DBLP:conf/crypto/GarayJM99} this appeared to be a limitation and only the status of a single contract was modeled, providing a manual proof to justify the correctness of this abstraction. 
The AVISPA platform \cite{DBLP:conf/cav/ArmandoBBCCCDHKMMORSTVV05} bounds the number of steps of honest agents which is often fine for finding attacks, but gives limited guarantees for verification.
This can work well for protocols based on public key cryptography, but runs into problems with several authentication and contract protocols \cite{DBLP:conf/crypto/GarayJM99,PKCS11standard,yubikeymanual}. 

Moreover, a number of unbounded-session automated verification tools \cite{DBLP:conf/sp/KremerK14,DBLP:conf/cav/MeierSCB13,DBLP:conf/csfw/Blanchet01} either make use of abstraction to enforce decidability, or allow for the possibility of non-termination.
% StatVerif tool by Arapinis \etal \cite{DBLP:conf/csfw/ArapinisRR11} propose an extension of the applied pi calculus, which is translated to Horn clauses and analyzed by the ProVerif tool. Their translation is sound but limits the scope of protocols that can be analyzed. Moreover, StatVerif can only handle a finite number of protocol sessions and is limited to the verification of secrecy properties.
For example, the ProVerif tool \cite{DBLP:conf/csfw/Blanchet01} uses an abstraction that encodes protocols in Horn clauses to avoid the exploration of the state space of a verifications system. 
The abstraction is efficient because it avoids the common state-explosion of protocol verification and it does not require a limitation to bounded sessions. 
While this works fine for many protocols \cite{DBLP:conf/csfw/KustersT09,DBLP:conf/post/ChevalB13,DBLP:conf/post/ChothiaSS15}, it lacks support for protocols which maintain long term global states \cite{DBLP:conf/crypto/GarayJM99,PKCS11standard,yubikeymanual}. 
This state is not local to a session: if one session updates the state, then it is updated for other sessions too. 
For these stateful protocols, ProVerif models an ever-increasing set of facts representing attacker knowledge, and is not able to associate those facts with the states in which they arose. 
For this reason, the tool typically reports many false attacks \cite{DBLP:conf/csfw/ArapinisRR11,DBLP:conf/csfw/BruniMNN15}. 


Another verification approach that supports the automated verification of protocols with unbounded sessions is the Tamarin prover \cite{DBLP:conf/cav/MeierSCB13,DBLP:conf/sp/KremerK14}. 
Instead of abstraction techniques, it uses backward search and lemmata that allow to cut of search to cope with the infinite state spaces. 
The benefit of Tamarin \cite{DBLP:conf/cav/MeierSCB13} and related tools \cite{DBLP:conf/sp/KremerK14} is a great amount of flexibility in formalising relationships between data that cannot be captured by a particular abstraction approach.
However it comes at the price of loosing automation, \ie, that the user has to supply insight into the problem by proving auxiliary lemmata.
Even for quite simple stateful protocols \cite{DBLP:conf/ccs/Modersheim10}, such lemmata have to be supplied by the user to achieve termination.
% This extension can be used for reasoning on stateful protocols \cite{yubikeymanual} , \cite{PKCS11standard} , \cite{DBLP:conf/crypto/GarayJM99}, but its user may need to interact with the verifier to add lemmatas.


% If the proof strategy chooses the wrong proof step in one case, it will always choose the same wrong proof step in the same situation, which takes a lot of human effort to understand the protocol and manually add lemmatas that allow to cut of search to cope with the infinite state spaces.
% Even for quite simple stateful protocols, such lemmatas have to be supplied by the user to achieve termination.


% Our work
In this paper, we propose a fully automated security protocol verification framework.
Our key insight is that human experts verify protocols using their experience in proving protocols.
Instead of trying every possible proof step in one case like the amateurs, they choose the most appropriate proof step based on their observation on current proof state and proof history.
There have been various stateful protocol verification examples \cite{DBLP:journals/jcs/DelauneKS10,DBLP:journals/jar/Guttman12,DBLP:journals/jcs/Wang06} using hand proof.
% Besides, much progress 
% \cite{DBLP:books/lib/HastieTF09},
% \cite{DBLP:journals/nature/LeCunBH15},
% \cite{DBLP:conf/nips/KrizhevskySH12},
% \cite{DBLP:conf/cvpr/HeZRS16}
% towards artificial intelligence has been made using supervised learning systems that are trained to replicate the decisions of human experts.
If the verification system can learn the human experts' proof strategy using machine learning algorithms during the verification progress, it can achieve automated verification of stateful protocols.



However current machine learning algorithms 
\cite{DBLP:books/lib/HastieTF09,DBLP:journals/nature/LeCunBH15,DBLP:conf/nips/KrizhevskySH12,DBLP:conf/cvpr/HeZRS16}
are not applicable to assist protocol verification. 
Firstly, these algorithms have required large amounts of hand-labelled training data and current protocol verification tools cannot generate such amounts of proof data.
On the other hand, these algorithms must be able to learn from a direct association between actions and rewards.   
However, this delay in protocol verification, which can be hundreds of timesteps long, seems particularly daunting and reduces the learning result. 
Another issue is that these algorithms assume the data samples to be independent, while in protocol verification one typically encounters sequences of highly correlated states. 


To overcome these challenges, we introduce two contributions.
% Our vision is that in the interactive mode .
% In detail, the framework contains two parts:
% \textbf{1) Discovering features from historical proof data.}
\textbf{Firstly}, we first introduce reinforcement learning, in particular Deep Q Learning (DQN) \cite{DBLP:journals/corr/MnihKSGAWR13}, into protocol verification.
Reinforcement learning systems are trained from their own experience, in principle allowing them to exceed human capabilities, and to operate in protocol verification where human expertise is lacking.
Besides, to alleviate the problems of correlated data and dependent distributions, DQN uses an experience replay mechanism \cite{lin1993reinforcement} which randomly samples previous transitions, and thereby smooths the training distribution over many past behaviors.

% \textbf{2) Proving security protocols using reinforcement learning.}
\textbf{Secondly}, we propose a fully automatically protocol verification framework for security protocols, especially stateful security protocols.
Using the tamarin prover as a backend tool, this framework can analyze protocols without bounding the number of sessions, nor making any abstractions. 
Instead of applying the original simple proof strategy of tamarin prover, we use a smart proof strategy learned by DQN to verify security properties in security protocols.
We illustrate the framework on several stateful protocols \cite{DBLP:conf/crypto/GarayJM99,PKCS11standard,yubikeymanual} and it can automated verify several stateful protocols such as Yubikey protocol \cite{yubikeymanual} which state-of-the-art verification tools cannot verify automatically.
% Contributions
% The contributions of the paper are as follows:

% We propose a tool for analyzing protocols that may involve non-monotonic global state. As a result, relying on the tamarin prover, we can analyze protocols without bounding the number of sessions, nor making any abstractions. 
% We illustrate the tool on several case studies: a complex case study of the Yubikey security device, as well as several examples analyzed by other tools that aim at analyzing stateful protocols.

% We show that the verification strategy based on DQN adapt to most stateful protocols and it can automated verify several stateful protocols such as Yubikey protocol which state-of-the-art verification tools cannot verify automatically.

% \begin{enumerate}
% 	\itemsep=4mm

% 	\item We designed the first general framework of formally modeling and verifying security protocols using crowdsourcing.
% 	\item We proposed and implemented for crowdsourcing participants to model and analyze security protocols, while also automatically translates the models into clauses verifiable by Tamarin Prover.
% 	\item We formally verified various protocols which state-of-the-art methods cannot prove and fixed the weaknesses.

% \end{enumerate}


==> s-casestudy.tex <==
%!TEX root =s-verifywithrl.tex
\section{Case Study} % (fold)
\label{sec:casestudy}

In this section we briefly overview some of the case studies we performed. 
These case studies include the Yubikey protocol ...

For each of the case studies we provide the number of typing lemmas that were needed by the tamarin prover and whether manual guidance of the tool was required. 

The Yubikey is a small hardware device designed to authenticate a user against network-based services. Manufactured by Yubico, a Swedish company, the Yubikey itself is a low cost (\$25), thumb-sized USB device. In its typical configuration, it generates one-time passwords based on encryptions of a secret value, a running counter and some random values using a unique AES-128 key contained in the device. The Yubikey authentication server accepts a one-time password only if it decrypts under the correct AES key to a valid secret value containing a counter larger than the last counter accepted. The counter is thus used as a means to prevent replay attacks. To date, over a million Yubikeys have been shipped to more than 30,000 customers including governments, universities and enterprises, \eg Google, Microsoft, Agfa and Symantec. 



==> s-dqn.tex <==
%!TEX root =s-verifywithrl.tex
\section{Verification module}
\label{sec:dqn}

Briefly, the Verification module selects a proof path from the verification tree.
The selection is guided by the DQN.
Then, we determine the correctness of the selection by the DQN.
We present details of our DQN in \Cref{subsec:dqn}.
In \Cref{subsec:correctness}, we describe our method of correctness determination.

% The determination result either presents a successful or failed verification, or leads to a generation of subtree.

\subsection{Deep Q Network}
\label{subsec:dqn}

% Reinforcement Learning is a commonly used framework for learning control policies in environments. 
% The environment can be formulated as a sequence of state transitions $(s, a, r, s')$ of a Markov Decision Process (MDP). 
% The agent takes an action $a$ in state $s$ by consulting a state-action value function $Q(s, a)$, which is a measure of the action's expected long-term reward. 
% Q-Learning is a model-free technique which is used to learn an optimal $Q(s, a)$ for the agent. Starting from a random Q-function, the agent continuously updates its Q-values by playing the game and obtaining rewards. 
% The iterative updates are derived from the Bellman equation:

% \begin{equation}
% Q_{i+1}(s,a) = E[r + \gamma\ \underset{{a}'}{max}Q_{i}({s}',{a}')\mid s,a]
% \end{equation}


\begin{algorithm}  
\caption{Deep Q-learning Algorithm}  
\label{alg:dql}  
\begin{algorithmic}[1] 
\STATE{Initialize replay memory $D$ to capacity $N$}
\STATE{Initialize action-value function $Q$}
\REPEAT
\STATE{Initialize proof state $s_1$}
\LOOP
\STATE{Compute current state $s_t$}
\STATE{With probability $\epsilon$ select a random action $a_t$}
\STATE{otherwise select $a_t = max_a Q(s_t, a; \theta)$}
\STATE{Generate proof path from $a_t$}
% \IF{loop detected}
\STATE{Observe reward $r_t$ and state $s_{t+1}$}
\STATE{Store transition $(s_t, a_t, r_t, s_{t+1})$ in $D$}
\STATE{Sample random minibatch of transitions $(s_j, a_j, r_j, s_{j+1})$ from $D$}
\STATE{Set $y_j = r_j + \gamma max_{{a}'}Q(s_{j+1},{a}';\theta)$}
\STATE{Perform a gradient descent step on $(y_j - Q(s_j, a_j; \theta))^{2}$}
\ENDLOOP
\UNTIL{verification success}
\end{algorithmic}  
\end{algorithm} 

There are two main reasons for introducing DQN to \ourtool:
1) Compared with supervised learning algorithms, the DQN does not require any proof data of various protocols and prior knowledge for training.
It optimizes itself according to its experience
which is suitable for protocol verification.
2) As proved in Appendix~\ref{sec:proof_of_our_insight}, we have an insight that a supporting lemma is on
the incorrect path with lower probability, when a random strategy is given.
Since the DQN generally requires a reward for evaluating its selection and optimizing itself,
we transform the correctness of a proof path into rewards of all the nodes on the path.
Note that the DQN requires a reward which corresponds to a determined occurrence of an event.
In our case there is no such occurrence.
Instead, we leverage probability of the path's correctness to construct rewards.
Optimizing with the reward, the DQN is able to select a supporting lemma with higher probability.
% The initial strategy in DQN is purely random.
% After the strategy is sufficiently optimized, it can smartly choose the supporting lemma with a higher probability.


In \ourtool, the DQN selects a path by iteratively inputting a state and outputting the choice of the next node, and it optimizes itself according to the collected incorrect selected paths.
Specifically, the input state $s$ of the DQN is transformed from information in nodes, \ie, the constraint reduction rule and the step.
Since the network is optimized by the reward of its historical selection,
it is important that the states of different nodes in the tree are identical.
As shown in \Cref{fig:tree} (c), the rule in the tree may be the same, \ie, rule $!KU(h(k))@\#vk$ occurs both at depth 2 and 3.
Hence, we provide the position of the node to the network.
The output of the DQN is an action number $a$, which corresponds to a child node.
It states that the network estimates a child node that may be the supporting lemma according to the current strategy.
The reward $r$ of an action is transformed from the output of correctness determination submodule.
In each epoch, there are two kinds of rewards.
1) The path may trap into an infinite loop, which is considered as incorrect.
We set the rewards of all the nodes on the path as the same negative numbers.
2) The path is correct.
Since we achieve a successful verification of the protocol, we set the rewards of all the nodes on the path as the same positive numbers.
Note that it is unnecessary to pass the positive rewards to the DQN in this case.
For research purpose, we optimize the DQN using these rewards to generate a smarter strategy,
which can be used to find a correct but shorter proof path.




% The reason that we introduce DQN is that the collected paths can be leveraged as a reward for guiding the optimization due to our insight, which is illustrated in \Cref{sec:evaluation}, and proved in Appendix~\ref{sec:proof_of_our_insight}.


In detail, we use the DQN with parameters $\theta$.
The action is chosen based on a strategy, generally expressed by $\pi$. 
The goal of the DQN is to find an optimal strategy that maximizes the rewards of supporting lemmata among the siblings. 
It starts with a random strategy to get a series of samples which contain states, actions and rewards: $\{(s_{1},a_{1},r_{1}),...(s_{t} , a_{t}, r_{t})\}$.
These samples are given to the network to optimize its strategy $\pi$.
The key feature of the DQN is the action value function $Q^{\pi}(s,a)$.
It represents the prediction value of an action $a$ in a state $s$.
Given a state $s$, the network calculates each action $a$'s prediction value $Q^{\pi}(s,a)$,
and chooses the action with the largest $Q$ value.
The optimization of the network is the process of updating the function $Q^{\pi}(s,a)$.
The update follows a principle: if the chosen action $a_{i+1}$ after performing an action $a_{i}$ brings more value, the value of current action $a_{i}$ should be updated to a higher value.


In order to find the best possible action-value function, we use two strategies: 1) a greedy strategy to choose the action which may have the largest $Q$ value currently;
2) an exploration strategy to choose random actions, which is to explore the values of unchosen actions, which will update the $Q$ value and obtain a better strategy. Combining the two strategies, we use a $\epsilon$-greedy strategy to select actions. Here, $\epsilon$ is a probability value for selecting random actions.
We change the value of $\epsilon$ to get different exploration ratios.

The update of the action-value function relies on a loss function $L(\theta_i)$.
Here, $\theta_i$ is the network's parameters at epoch $i$.
In our case, the loss function is the deviation of the reward given by Verification module and the prediction reward of the network.
We make the standard assumption that future rewards are discounted by a factor of
$\gamma$ per time-step.
The optimal action-value function obeys an intuition: at iteration $i-1$, if the optimal value $Q({s}',{a}',\theta_{i-1})$ of the state ${s}'$ at the next time-step was known for all possible actions ${a}'$, then the optimal strategy is to select the action ${a}'$ maximizing the expected value of $r + \gamma \underset{{a}'}{max}Q({s}',{a}',\theta_{i-1})$.
We update the parameters of network by back-propagation using gradient descent.
Therefore, the loss function we use in our network is as follows, where $r + \gamma \underset{{a}'}{max}Q({s}',{a}',\theta_{i-1})$ is optimal value of action $a$ and $Q(s,a,\theta_i)$ is current value of $a$.

\begin{align}
L(\theta_i) = \mathds{E}[(r + \gamma \underset{{a}'}{max}Q({s}',{a}',\theta_{i-1}) - Q(s,a,\theta_i))^{2}]  \nonumber
\end{align}

Moreover, we utilize a technique known as experience replay \cite{lin1993reinforcement} where we store the experiences at each epoch, $e_t = (s_t, a_t, r_t, s_{t+1})$
in a data-set $D = \{e_1, ..., e_N\}$, pooled over many epochs into a replay memory.
At each epoch of verification process, we apply network updates with samples of experience.
In practice, our network only stores the last $N$ experience tuples in the replay memory,
where $N$ is 100 in our implementation.

This approach has two advantages.
First, each reward of a selection in an epoch is potentially used in network optimization in many epochs afterwards, which allows for greater data efficiency.
In each epoch, the DQN selects a path and optimizes itself according to the correctness of the path.
In our case, there is a limited amount of selection experiences in each epoch, which is transformed to a low quantity of training samples.
Adopting experience replay, we repeatedly use the training samples in many epochs, which efficiently increases the convergence rate.
Second, randomizing the samples breaks the correlations in selections by the DQN and therefore we generate a smarter strategy.
In our case, the DQN selects a path by iteratively inputting a state and outputting the choice of the next node.
If the path is estimated incorrect,
the reward of each selection is set to a negative reward.
There may be a case that though the supporting lemma is selected in a step,
the DQN selects a child node which leads to non-termination in next steps.
If the DQN learns all the samples in a epoch, it may consider that the selection of supporting lemma is incorrect.
Hence, we sample the training data to reduce the probability of divergence.

% learning directly from consecutive samples is inefficient, owing to the strong
% correlations between the samples; randomizing the samples breaks these correlations and therefore reduces the variance of the updates

% the training sample distribution is averaged over many epochs, which smooths out learning and avoids divergence in the parameters.
% In our case, updating the parameters in current epoch directly influences the selections by DQN in next epochs.
% For example, if the action with the largest prediction value is the left child node then the training samples will be dominated by samples from the left-hand side;
% If the action switches to right child node in tree then the training distribution will also switch.
% If we simply use training sample in current epoch to optimize the network, the parameters could get stuck in a poor local minimum.




\subsection{Correctness Determination}
\label{subsec:correctness}


We determine the correctness of selected paths to give the DQN a reward for its selection path.
In detail, we detect whether there are large amounts of loops in the path.
This method is motivated by an observation in historical proof data.
In this data, we discovered that several non-termination cases are caused by the loops in automated protocol analysis.
% Briefly, proof paths chosen by DQN can be divided into three categories.
% 1) The path is estimated incorrect: it states that the path may lead to a non-termination verification.
% 2) The path is estimated correct but incomplete: it states the path is estimated correct, but it is incomplete.
% Hence, it requires a longer path to fully determine its correctness.
% 3) The path is correct and complete: it states that we have successfully verify the protocol using this path.


\begin{figure}[htbp]
\centering
\includegraphics[scale=0.3]{a.jpg}
\caption{An example of verification loop.}
\label{fig:infinite-loop}
\vspace{-0.1in}
\end{figure}

\Cref{fig:infinite-loop} shows an example of verification loop which tamarin encounters.
Words in blue indicate a choice by tamarin prover, and words in black indicate a tag in verification.
In this example, tamarin prover makes five choices, which begins with:
\begin{align}
!\kwe{KU(\ aenc(< '2', ~ni.1, nr.1, \$R.1>,\ pk(~ltkA.1)))\ @\ \#vk.1\ ) } \nonumber
\end{align}
Each choice is similar to the former one.
We consider this proof incorrect since the loop in it leads to a non-termination result.
However, there are several kinds of loops.
The loop shown above, where each step is similar, is the most common one.
There exists a loop in a sequence like $[a, b, a, b, ...]$ or $[a, b, c, a, b, c, ...]$, where $a,b$ are constraint reduction rules.
Simply comparing each node's information is not effective.
Moreover, the information of node in a path contains a constraint reduction rule.
As shown in \Cref{fig:infinite-loop}, there are variables $ni.1, ni.2, ni.3$ in these rules.
Note that tamarin prover appends the variable in the rule with a number to distinguish the different states.
These variables are not same, but the rules are similar.
Based on this observation, we should detect the similarity of the rules.

Hence, we use the algorithm below to detect the loops.
In the algorithm, we check the sequence $(s_{1}, s_{2},..., s_{k})$ in multiple rounds.
Moreover, this algorithm is executed after 20 rounds to increase our efficiency.
First, we generate several subsequences from rule $s_{k}$ with a distance of $1$ to $k-1$.
For each subsequence, we detect the similarity of each rule and another one.
Here we use levenshtein distance to detect similarity.
The distance between two rules $x$ and $y$ is the minimum number of single-character edits (insertions, deletions or substitutions) required to change rule $x$ into rule $y$.
If the distance between $x$ and $y$ is less than 10\% of the rule $x$, we assume these two rules are similar.
When there exist more than three similar rules in a subsequence, we find a loop.
Once all subsequences are checked and no loops are found, the path is estimated to be correct.
% This distance fits in situations where a small number of differences is to be expected. 
% Note that we determine the incorrectness every five rounds after ten rounds to increase our efficiency.

\begin{algorithm}  
\caption{Loop Detection Algorithm}  
\label{alg:similarity}  
\begin{algorithmic}[1] 
\REQUIRE $(s_{1}, s_{2},..., s_{k})$ \COMMENT{a string sequence, where each element represents a constraint reduction rule}
\IF{$k \geq \alpha$}
\FOR{$j=1$ to $k-1$}
\STATE $count = 0$
\STATE $S = (s_{k}, s_{k-j}, s_{k-2j},...)$ 
\FOR{each element $x$ in $S$}
\FOR{each element $y$ in $S$}
\IF{$x \neq y$}
\STATE $n$ = length of $x$, $m$ = length of $y$
% \STATE Initialize vector $v[n+1]$
\FOR{$a=1$ to $n$}
\FOR{$b=1$ to $m$}
\IF{$y[a]==x[b]$}
\STATE $cost=0$
\ELSE
\STATE $cost=1$
\ENDIF
\STATE  $v[b] = \textup{min}\left\{\begin{matrix}
v[b-1] + 1\\ 
b\\ 
b-2 + cost
\end{matrix}\right.$
\ENDFOR
\ENDFOR
\IF{$v[m] / m$ $< \beta$ }
\STATE $count = count + 1$ 
\ENDIF
\ENDIF
\ENDFOR
\ENDFOR
\IF{$count$ $\geq \gamma$ }
\RETURN TRUE 
\ENDIF
\ENDFOR
\RETURN FALSE 
\ELSE
\RETURN FALSE 
\ENDIF
\end{algorithmic}  
\end{algorithm}  



If the path is estimated to be correct, we use tamarin prover to check whether it is complete.
If tamarin prover leads to a successful verification with the path,
we assume the path is correct and complete.
In this case, we can terminate \ourtool.
If tamarin prover states that the proof process is incomplete and there are more rules to be selected,
we assume the path is incomplete and expand the verification tree to extend the path in the next round.


==> s-features.tex <==
%!TEX root =s-verifywithrl.tex
\section{Features} % (fold)
\label{sec:features}

\textbf{1) Proof method ranking strategy used by tamarin}

There are several proof methods in a protocol verification step. 
The order of solving them has a significant impact on the size of the generated proofs and therefore the runtime of the algorithm. 
We currently use a very simple proof method ranking strategy.
Whenever possible, we apply a proof method that is guaranteed not to result in a case distinction;
Otherwise, we use the first applicable method from the list,
which contains the methods that may result in a case distinction.
We use the following heuristic to delay the solving of proof method that are unlikely to result in a contradiction. 
We delay solving a goal $p$ requiring a message $m$, if $m$ does not contain a variable of sort fresh or if $m$ can be extracted using projection and inversion from a message sent by a protocol step that does not occur later than $p$. 
Intuitively, we delay solving such premises because the adversary is likely to be able to construct their required messages.

\textbf{2) Proof method similarity feature}

In historical proof data, we discovered that several non-termination cases are caused by the loops in automated protocol analysis.

\begin{figure}[htbp]
\centering
\includegraphics[width = .5\textwidth]{a.jpg}
\caption{An infinite verification loop in automated protocol analysis}
\label{fig:infinite-loop}
\end{figure}

As shown in \Cref{fig:infinite-loop}, Tamarin prover keeps solving a goal 
\begin{align}
\kwe{KU(\ aenc(<'2', ~ni, nr, \$R>,\ pk(~ltkA)))\ @\ \#vk\ ) } \nonumber
\end{align}
similar to the former ones.
Based on these observations, we delay solving such cases which may lead to non-termination cases by \Cref{alg:similarity}.

\begin{algorithm}  
\caption{Loop detection algorithm}  
\label{alg:similarity}  
\begin{algorithmic}  
\REQUIRE $(s_{1}, s_{2},..., s_{k})$ \COMMENT{proof path}
% \STATE $S \leftarrow (s_{1}, s_{2},..., s_{k})$ \COMMENT{proof path}
\FOR{$i=1$ to $k-1$}
\IF{$s_{i} = s_{i+1}$} 
\RETURN loop found 
\ENDIF
\ENDFOR
\FOR{$i=1$ to $k-1$}
\STATE $S \leftarrow (s_{k}, s_{k-i}, s_{k-2i},...)$ 
\IF{duplicate elements in S $\geq$ 4}
\RETURN loop found 
\ENDIF
\ENDFOR
\end{algorithmic}  
\end{algorithm}  




==> s-verifywithrl <==
\Changes@AuthorID1 ;\Changes@AuthorColor \Changes@AuthorID1 \endcsname ;\Changes@AuthorName \Changes@AuthorID1 \endcsname ;0\Changes@AuthorID1 \endcsname ;0\Changes@AuthorID1 \endcsname ;0\Changes@AuthorID1 \endcsname 
\Changes@AuthorID2 ;\Changes@AuthorColor \Changes@AuthorID2 \endcsname ;\Changes@AuthorName \Changes@AuthorID2 \endcsname ;0\Changes@AuthorID2 \endcsname ;0\Changes@AuthorID2 \endcsname ;0\Changes@AuthorID2 \endcsname 

